Unlocking Efficient, Scalable, and Continual Knowledge Editing with Basis-Level Representation Fine-Tuning

Large language models (LLMs) have achieved remarkable performance on various natural language tasks. However, they are trained on static corpora and their knowledge can become outdated quickly in the fast-changing world. This motivates the development of knowledge editing methods designed to update certain knowledge in LLMs without changing unrelated others. To make selective edits, previous efforts often sought to update a small amount of parameters in some specific layer(s) of a LLM. Nonetheless, in challenging scenarios, they still fall short in making successful edits while preserving knowledge irrelevant to the updates simultaneously, resulting in a notable editing-locality trade-off. In this work, we question if the trade-offs are caused by the fact that parameter-based updates have a global effect, i.e., edited parameters affect all inputs indiscriminately. In light of this, we explore the feasibility of representation fine-tuning, which applied some linear update to a few representations in a learned subspace, for knowledge editing. While being effective to enhance an LLM's general ability as demonstrated in the previous work, we theoretically show that this linear update imposes a tension in editing-locality trade-off. Subsequently, BaFT is proposed to break the linearity. BaFT computes a weight for each basis that spans a dimension of the subspace based on the input representation. This input-dependent weighting mechanism allows BaFT to manage different types of knowledge in an adaptive way, thereby achieving a better editing-locality trade-off. Experiments on three LLMs with five editing benchmarks in diverse scenarios show the superiority of our method.

==> subfiles/4_experiment_backup.tex <==
\section{Experiment}
\label{sec:experiment}


In this section we experiment the proposed {\name} for knowledge editing on three 7B-level language models (LMs) over five benchmarks.  
{\name} shows competitive performance with much less parameters, thereby achieving notable parameter efficiency. 


\subsection{Experiment Setup}


\textbf{Base Models.}
We conduct experiments on three representative autoregressive LLMs from different model families. \textbf{LLaMA 2-7b} and \textbf{LLaMA 2-7b-Chat} \citep{touvron2023llama} have been widely studied in the literature \citep{} and we follow this convention. Trending \textbf{LLaMA 3-8b-Instruct} \citep{} and \textbf{Gemma 1.1-7b-Instruct} \citep{} are also studied. 



\textbf{Tasks.}
Following previous works \citep{}, 
we edit emerging and counterfactual knowledge: WikiData\sub{recent}, WikiData\sub{counterfact} \citep{}, WikiBio \citep{}, ConvSent \citep{}, and ZsRE \citep{}. 
\tc{Due to page limitation, we defer more details about these datasets to Appendix \ref{app:data}.}
% \tc{Hallucination}. 
We consider different editing scenarios.
\textbf{Single Editing} updates one piece of knowledge at a time. \textbf{Continual Editing} and \textbf{Batched Editing}, on the other hand, update multiple pieces of knowledge in a sequential or batched way. Note that the latter two scenarios are more challenging due to the catastrophic forgetting \citep{} and potential knowledge conflicting \citep{} as observed in the literature. 



\textbf{Baselines.}
We follow \cite{} and choose AdaLoRA \citep{}, ROME and FT-L \citep{meng2022locating}, and MEMIT \citep{meng2022mass} as baselines. 
In continual editing scenarios, we further include representative memory-based methods GRACE \citep{} and WISE \citep{wang2024wise}. 
All these baselines, same as ours, \textit{do not require a larges-scale hard-to-access training data, or training additional models}:
AdaLoRA learns a low-rank update for model parameters on the new knowledge while keeping less important parameters unchanged, thereby achieving a highly efficient and precise PEFT.
ROME applies a causal-tracing analysis to identify the layer wherein the knowledge is stored and then solves an analytic rank-one update. FT-L, on the other hand, directly finetunes the layer identified by ROME with an additional KL divergence loss. MEMIT extends ROME to a batched editing setting by identifying a series of layers to edit and finding the updates through least squares solutions\footnote{Due to the substantial difference between LLaMA and Gemma architectures, existing MEMIT implementations optimized for LLaMA family cannot be applied to Gemma so we omit testing MEMIT on Gemma.}. 
GRACE and WISE are specialized for continual editing. They leverage side parameters to save new knowledge and learn gating mechanism to determine whether pre-trained or new knowledge should be used during inference. 
% Notably, the parameters number in these methods can grow with time and is significantly larger than ours. 
Finally, we include ReFT as a baseline that uses a subspace of same rank as {\name}. 
% We assign ReFT with the total subspace rank the same as {\name}. 
We report hyper-parameters of different methods in Appendix \ref{app:hparams}.

%     \item 
%     \item \textbf{FT-L} directly fine-tunes a particular subset of model parameters  \citep{meng2022locating}.
%     \item \textbf{Locate-and-Edit} paradigm 
%     ROME applies a causal-tracing to identify the layer wherein the knowledge is stored and then learns a rank-one update. FT-L, on the
% other hand, directly finetunes the layer identified by ROME. Recently, MEMIT extends
% ROME to a large-scale setting, where the edits can be made more efficiently.
%     ROME and MEMIT locate the neurons or (a few) layers wherein the new knowledge is stored based on causal tracing, and update these parameters in an analytic way or with a regression problem \citep{meng2022locating, meng2022mass}.    
%     \item \textbf{Memory-based} methods such as GRACE and WISE store new knowledge with side parameter groups and retrieve proper groups during inference \cite{, wang2024wise}. 
% \end{itemize}
% Notably, all baselines do not require a larges-scale hard-to-access data or training additional models. 




\textbf{Evaluation.}
We evaluate the editing performance from multiple aspects as in previous works \cite{}. Given an edited model,
\textbf{reliability (Rel.)} evaluates whether its successfully learns the new knowledge;
\textbf{generality (Gen.)} measures to what extent it can generalize to rephrased knowledge inquiries;
\textbf{locality (Loc.)} quantifies how much the model can retain its original output on irrelevant knowledge inquiries;
\textbf{portability (Por.)} checks if the model is able to transfer new knowledge to related content.
For a more comprehensive comparison, we follow \citet{} and report the average of different metrics. 



\subsection{Single Editing Performance}

In this section, we evaluate the effectiveness of the proposed {\name} for conducting Single Editing on 
WikiData\sub{recent}, WikiData\sub{counterfact} \citep{}, WikiBio \citep{}, and ConvSent \citep{}. 
Convsent benchmark only supports LLaMA family. 
Moreover, as all baseline methods were only tested on LLaMA 2 in existing works and there is no public recommended hyperparameter configuration for LLaMA 3-8b-Instruct and Gemma 1.1-7b-Instruct, we conducted a hyperparameter tuning with similar efforts as for our method. \tc{However, due to the significant difference between LLaMA and Gemma architecture, ROME can only be applied when finetuning Gemma on small Wiki\sub{recent} and Wiki\sub{counterfact}, and MEMIT ...}
The four benchmarks do not contain proper irrelvanet data. Consequentially, {\name} does not involve the locality regularization. 

Results of Single Editing using different methods are reported in Table \ref{tab:single}. 
According to the table, the proposed {\name} and its simplified form ReFT achieved highly competitive performance of editing three LLMs on four datasets, 
and {\name} is capable of achieving consistently better locality than ReFT with no or minimal degradation of the editing effectiveness. 
In contrast, other baselines suffer from failing to achieve high edit success rate or maintaining good locality. 
In addition, these methods showed significant performance gaps when editing different base models even after we tuned hyperparameters such as layer
These results clearly demonstrates the effectiveness of {\name} (and ReFT) as a new promising direction for knowledge editing. 


\begin{table}[htbp]
\centering
% \small
\caption{
Performance comparison of Single Editing using different methods on four benchmark datasets. 
Results marked with ``$\heartsuit$'' are taken from \citet{zhang2024comprehensive}, and ``\xmark'' indicates no proper compatible implementation is avaiable. 
ConvSent benchmark only supports LLaMA family. 
% ZsRE results are reported in the next section. 
}
\label{tab:single}
\resizebox{\linewidth}{!}{%{}
\begin{tabular}{l cccc c cccc c ccc c c}
\toprule
& \multicolumn{4}{c}{Wiki\sub{recent}} && \multicolumn{4}{c}{Wiki\sub{counterfact}} && \multicolumn{3}{c}{WikiBio} && {ConvSent} \\




% \midrule
\cmidrule{1-16}
\multicolumn{16}{c}{LLaMA 2-7b-chat} \\
\cmidrule{2-16}
% \midrule
& Rel. & Por. & Loc. & Avg. && Rel. & Por. & Loc. & Avg. && Rel. & Loc. & Avg. && Rel. \\
% & \multicolumn{4}{c}{Wiki\sub{recent}} && \multicolumn{4}{c}{Wiki\sub{counterfact}} && \multicolumn{3}{c}{WikiBio} && \multicolumn{3}{c}{Convsent} \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-14} \cmidrule{16-16}
AdaLoRA$^\heartsuit$ & 0.66 & 0.47 & 0.56 & 0.56 && 0.70 & 0.53 & 0.72 & 0.65 && 0.97 & 0.58 & 0.78 && 0.45 \\
FT-L$^\heartsuit$    & 0.71 & 0.49 & 0.64 & 0.61 && 0.51 & 0.39 & 0.63 & 0.51 && 0.66 & 0.60 & 0.63 && 0.50 \\
ROME$^\heartsuit$    & 0.85 & 0.37 & 0.66 & 0.63 && 0.83 & 0.39 & 0.65 & 0.62 && 0.95 & 0.47 & 0.71 && 0.46 \\
MEMIT$^\heartsuit$   & 0.85 & 0.37 & 0.66 & 0.63 && 0.83 & 0.40 & 0.64 & 0.62 && 0.94 & 0.52 & 0.73 && 0.45 \\
\cdashline{2-16}\noalign{\vskip 0.5ex}
ReFT                 & 1.00 & 0.72 & 0.61 & 0.78 && 1.00 & 0.77 & 0.53 & 0.77 && 1.00 & 0.93 & 0.97 && 1.00 \\
{\name} (Ours)       & 1.00 & 0.73 & 0.61 & 0.78 && 1.00 & 0.78 & 0.53 & 0.77 && 1.00 & 0.94 & 0.97 && 1.00 \\





\cmidrule{1-16}
\multicolumn{16}{c}{LLaMA 3-8b-Instruct} \\
\cmidrule{2-16}
& Rel. & Por. & Loc. & Avg. & & Rel. & Por. & Loc. & Avg. && Rel. & Loc. & Avg. && Rel. \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-14} \cmidrule{16-16}
AdaLoRA         & 1.00 & 0.43 & 0.61 & 0.68 && 1.00 & 0.25 & 0.55 & 0.60 && 1.00 & 0.42 & 0.71 && 1.00 \\
FT-L            & 0.47 & 0.25 & 0.27 & 0.33 && 0.44 & 0.10 & 0.27 & 0.27 && 0.56 & 0.39 & 0.48 && 0.52 \\
ROME            & 0.99 & 0.33 & 0.34 & 0.55 && 1.00 & 0.52 & 0.24 & 0.59 && 0.92 & 0.62 & 0.77 && 0.98  \\
MEMIT           & 0.99 & 0.32 & 0.34 & 0.55 && 0.99 & 0.49 & 0.24 & 0.57 && 0.04 & 0.08 & 0.06 && 0.32 \\
\cdashline{2-16}\noalign{\vskip 0.5ex}
ReFT            & 1.00 & 0.63 & 0.61 & 0.75 && 1.00 & 0.70 & 0.51 & 0.74 && 0.98 & 0.90 & 0.94 && 0.98 \\
{\name} (Ours)  & 1.00 & 0.65 & 0.61 & 0.75 && 1.00 & 0.72 & 0.53 & 0.75 && 0.97 & 0.93 & 0.95 && 0.96 \\





\cmidrule{1-16}
\multicolumn{16}{c}{Gemma 1.1-7b-Instruct} \\
% \cmidrule{2-18}
% \midrule
\cmidrule{2-16}
& Rel. & Por. & Loc. & Avg. && Rel. & Por. & Loc. & Avg. && Rel. & Loc. & Avg. && Rel. \\
% & \multicolumn{4}{c}{Wiki\sub{recent}} && \multicolumn{4}{c}{Wiki\sub{counterfact}} && \multicolumn{3}{c}{WikiBio} && \multicolumn{3}{c}{Convsent} \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-14} \cmidrule{16-16}
AdaLoRA         & 1.00 & 0.26 & 0.53 & 0.60 && 1.00 & 0.27 & 0.50 & 0.59 && 1.00 & 0.66 & 0.83 && \xmark  \\
FT-L            & 0.31 & 0.04 & 0.17 & 0.17 && 0.26 & 0.01 & 0.13 & 0.13 && 0.24 & 0.14 & 0.19 && \xmark  \\
ROME            & 0.65 & 0.23 & 0.33 & 0.40 && 0.67 & 0.19 & 0.28 & 0.38 && 0.49 & 0.31 & 0.40 && \xmark\\
% MEMIT           & /    &      &      & / && /    &      &      & / && \xmark & \xmark & \xmark && \xmark & \xmark & \xmark \\ 
\cdashline{2-16}\noalign{\vskip 0.5ex}
ReFT            & 1.00 & 0.61 & 0.50 & 0.70 && 1.00 & 0.70 & 0.41 & 0.70 && 0.98 & 0.83 & 0.91 && \xmark \\ 
{\name} (Ours)  & 1.00 & 0.64 & 0.50 & 0.71 && 1.00 & 0.73 & 0.41 & 0.71 && 0.97 & 0.84 & 0.91 && \xmark \\ 



\bottomrule
\end{tabular}
}
\end{table}



\subsection{Continual and Batched Editing Performance.}


In this section we study the more challenging scenarios where the editing is conducted in a continual or batched way. 
We follow existing works \citep{} and experiment different methods with LLaMA 2-7b (non-chat version as in \citet{}), LLaMA 3-8b-Instruct, and Gemma 1.1-7b-Instruct on ZsRE. 
We note that the state-of-the-art continual editing method WISE contains substantially larger parameter size and is much more computational expensive. 
For better comparison, we include WISE\sub{light}, a lightweight version of WISE that contains 1/8 learnable parameters of the original WISE to make its training affordable. 
We would like to highligh that WISE\sub{light} does not affect WISE editing mechanism 
\footnote{In essense, WISE finds an influential FFN layer of a LLM to conduct knowledge editing. For each new knowledge, WISE finetunes a small portion of \textit{randomly} selected parameters in this FFN layer. WISE\sub{light} randomly drops a certain portion of parameters from the selection procedure. 
}, and still contains much more learnable parameters than {\name} and ReFT.
Learnable parameters used in different editing methods, along with their time consumption is presented in Table \ref{tab:stat}. 



\textbf{Continual Editing Performance.}
Table \ref{tab:continual} presents the main results of continually editing 1000 pieces of knowledge using ZsRE in three LLMs.
Our method was capable of achieving the best editing performance while maintaining excellent locality on three LLMs from different families. 
In comparison, standard editing methods AdaLoRA, FT-L, ROME, and MEMIT, encountered considerable performance gaps on different LLMs. 
At the same time, all of these methods fall short in editing multiple pieces of knowledge that emerge sequentially. 
Recent methods GRACE and WISE that were designed for handling continual editing also suffered from failure on editing Gemma, possibly due to the difference between Gemma and LLaMA.
These methods may benefit from a more comprehensive hyper-parameter tuning on each different base LLM model. 
Nonetheless, their prolonged running time will make this process very expensive, if not unaffordable. 

When comparing two representation engineering methods, {\name} and ReFT, with each other, 
we note that as in Single Editing, {\name} can maintain, if not surpass, the editing ability of ReFT.
In addition, when the editing number $T$ increases, {\name} shows excellent robustness against catastrophic forgetting, a crucial challenge in LLM finetuning \citep{}, 
as indicated by its high locality in all scenarios.
These results clearly show the effectiveness of our proposed {\name} in handling continual editing. 
% We provide more detailed ablation study on {\name} to uncover its effectiveness. 



\begin{table}[htbp]
\centering
% \small
\caption{
Performance comparison of Continual Editing with different methods on ZsRE dataset. 
Results marked with ``$\heartsuit$'' are taken from \citet{wang2024wise}. 
Editing performance is evaluated after conducting $T$ times of editing sequentially. 
}
\label{tab:continual}
% \renewcommand{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%{}
\begin{tabular}{l cccc c cccc c cccc c cccc}
\toprule
& \multicolumn{4}{c}{$T=1$} && \multicolumn{4}{c}{$T=10$} && \multicolumn{4}{c}{$T=100$} && \multicolumn{4}{c}{$T=1000$} \\


% \midrule
\cmidrule{1-20}
\multicolumn{20}{c}{LLaMA 2-7b} \\
\cmidrule{2-20}
% \midrule
& Rel. & Gen. & Loc. & Avg. & & Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. \\
% & \multicolumn{4}{c}{Wiki\sub{recent}} && \multicolumn{4}{c}{Wiki\sub{counterfact}} && \multicolumn{3}{c}{WikiBio} && \multicolumn{3}{c}{Convsent} \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20}
AdaLoRA              & 1.00 & 0.90 & 0.92 & 0.94 && 0.39 & 0.38 & 0.50 & 0.42 && 0.06 & 0.06 & 0.06 & 0.06 && 0.00 & 0.00 & 0.00 & 0.00 \\
FT-L                 & 0.57 & 0.53 & 0.96 & 0.69 && 0.35 & 0.31 & 0.12 & 0.26 && 0.29 & 0.26 & 0.09 & 0.21 && 0.24 & 0.20 & 0.25 & 0.23 \\
% FT-L$^\heartsuit$    & 0.57 & 0.52 & 0.96 & 0.68 && 0.48 & 0.48 & 0.76 & 0.57 && 0.30 & 0.27 & 0.23 & 0.27 && 0.19 & 0.16 & 0.03 & 0.13 \\
% ROME$^\heartsuit$    & 0.85 & 0.80 & 0.99 & 0.88 && 0.64 & 0.62 & 0.75 & 0.67 && 0.23 & 0.22 & 0.04 & 0.16 && 0.01 & 0.01 & 0.00 & 0.01 \\
% MEMIT$^\heartsuit$   & 0.84 & 0.81 & 0.99 & 0.88 && 0.58 & 0.58 & 0.85 & 0.67 && 0.02 & 0.02 & 0.02 & 0.02 && 0.04 & 0.04 & 0.02 & 0.03 \\
ROME                 & 0.96 & 0.91 & 0.98 & 0.95 && 0.38 & 0.35 & 0.05 & 0.26 && 0.18 & 0.17 & 0.02 & 0.12 && 0.01  & 0.01 & 0.00 & 0.01 \\
MEMIT                & 0.95 & 0.90 & 0.99 & 0.95 && 0.11 & 0.11 & 0.06 & 0.09 && 0.04 & 0.04 & 0.02 & 0.03 && 0.04 & 0.04 & 0.02 & 0.03 \\
GRACE$^\heartsuit$   & 0.98 & 0.08 & 1.00 & 0.69 && 0.96 & 0.00 & 1.00 & 0.65 && 0.96 & 0.00 & 1.00 & 0.65 && 0.97 & 0.08 & 1.00 & 0.68 \\
WISE\sub{full}$^\heartsuit$    & 0.98 & 0.92 & 1.00 & 0.97 && 0.94 & 0.88 & 1.00 & 0.94 && 0.90 & 0.81 & 1.00 & 0.90 && 0.77 & 0.72 & 1.00 & 0.83 \\
WISE\sub{light}      & 0.95 & 0.83 & 1.00 & 0.93 && 0.93 & 0.74 & 1.00 & 0.89 && 0.83 & 0.73 & 0.99 & 0.85 && 0.49 & 0.47 & 1.00 & 0.65 \\
% WISE\sub{light}      & 0.86 & 0.74 & 1.00 & 0.87 && 0.86 & 0.76 & 1.00 & 0.87 && 0.74 & 0.66 & 0.99 & 0.80 && 0.49 & 0.47 & 0.99 & 0.65 \\
\cdashline{2-20}\noalign{\vskip 0.5ex}
ReFT                 & 1.00 & 0.95 & 0.94 & 0.96 && 0.90 & 0.85 & 0.88 & 0.87 && 0.78 & 0.74 & 0.83 & 0.78 && 0.58 & 0.56 & 0.73 & 0.62 \\
{\name} (Ours)       & 1.00 & 0.94 & 0.97 & 0.97 && 0.89 & 0.84 & 0.97 & 0.90 && 0.75 & 0.70 & 0.98 & 0.81 && 0.63 & 0.60 & 0.98 & 0.74 \\




\cmidrule{1-20}
\multicolumn{20}{c}{LLaMA 3-8b-Instruct} \\
\cmidrule{2-20}
& Rel. & Gen. & Loc. & Avg. & & Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20}
AdaLoRA              & 1.00 & 0.99 & 0.85 & 0.95 && 0.27 & 0.26 & 0.26 & 0.26 && 0.03 & 0.03 & 0.01 & 0.02 && 0.00 & 0.00 & 0.00 & 0.00 \\
FT-L                 & 0.51 & 0.52 & 0.68 & 0.57 && 0.25 & 0.20 & 0.03 & 0.16 && 0.19 & 0.16 & 0.02 & 0.12 && 0.16 & 0.14 & 0.01 & 0.10 \\
ROME                 & 0.99 & 0.96 & 0.96 & 0.97 && 0.07 & 0.07 & 0.01 & 0.05 && 0.03 & 0.03 & 0.01 & 0.02 && 0.03 & 0.03 & 0.00 & 0.02 \\
MEMIT                & 0.99 & 0.96 & 0.98 & 0.98 && 0.02 & 0.02 & 0.01 & 0.02 && 0.06 & 0.06 & 0.03 & 0.05 && 0.06 & 0.06 & 0.03 & 0.05 \\
GRACE                & 0.33 & 0.00 & 0.54 & 0.29 && 0.33 & 0.02 & 0.56 & 0.30 && 0.33 & 0.02 & 0.57 & 0.31 && 0.33 & 0.02 & 0.55 & 0.30 \\
WISE\sub{light}      & 0.95 & 0.91 & 0.99 & 0.95 && 0.82 & 0.76 & 1.00 & 0.86 && 0.63 & 0.57 & 1.00 & 0.73 && 0.39 & 0.37 & 1.00 & 0.59 \\
% WISE\sub{light}      & 0.95 & 0.90 & 0.96 & 0.94 && 0.88 & 0.83 & 0.91 & 0.87 && 0.71 & 0.64 & 0.97 & / && 0.53 & 0.51 & 1.00 & / \\
\cdashline{2-20}\noalign{\vskip 0.5ex}
ReFT                 & 1.00 & 0.97 & 0.93 & 0.87 && 0.90 & 0.84 & 0.87 & 0.87 && 0.68 & 0.61 & 0.74 & 0.68 && 0.48 & 0.45 & 0.64 & 0.52 \\
{\name} (Ours)       & 1.00 & 0.95 & 0.96 & 0.89 && 0.89 & 0.82 & 0.95 & 0.89 && 0.70 & 0.64 & 0.93 & 0.76 && 0.50 & 0.49 & 0.93 & 0.64 \\



\cmidrule{1-20}

\multicolumn{20}{c}{Gemma 1.1-7b-Instruct} \\
\cmidrule{1-20}
& Rel. & Gen. & Loc. & Avg. & & Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. && Rel. & Gen. & Loc. & Avg. \\
\cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20}
AdaLoRA              & 1.00 & 0.97 & 0.67 & 0.88 && 0.19 & 0.20 & 0.18 & 0.19 && 0.03 & 0.03 & 0.01 & 0.02 && 0.00 & 0.00 & 0.00 & 0.00 \\
FT-L                 & 0.28 & 0.33 & 0.09 & 0.23 && 0.14 & 0.06 & 0.00 & 0.07 && 0.07 & 0.04 & 0.00 & 0.04 && 0.05 & 0.04 & 0.00 & 0.03 \\
ROME                 & 0.65 & 0.62 & 0.84 & 0.70 && 0.00 & 0.00 & 0.00 & 0.00 && 0.00 & 0.00 & 0.00 & 0.00 && 0.00 & 0.00 & 0.00 & 0.00 \\
% MEMIT                & \\
GRACE                & 0.39 & 0.00 & 1.00 & 0.46 && 0.39 & 0.01 & 1.00 & 0.47 && 0.39 & 0.01 & 1.00 & 0.47 && 0.39 & 0.01 & 1.00 & 0.47 \\
WISE\sub{light}      & 0.99 & 0.96 & 1.00 & 0.98 && 0.90 & 0.84 & 0.99 & 0.91 && 0.79 & 0.71 & 0.95 & 0.82 && 0.48 & 0.42 & 0.98 & 0.63 \\
% WISE\sub{light}      & 1.00 & 0.95 & 1.00 & 0.98 && 0.91 & 0.84 & 1.00 & 0.92 && 0.75 & 0.65 & 0.99 & 0.80 && 0.39 & 0.35 & 0.99 & 0.58 \\
\cdashline{2-20}\noalign{\vskip 0.5ex}
ReFT                 & 1.00 & 0.86 & 0.91 & 0.92 && 0.92 & 0.81 & 0.81 & 0.85 && 0.66 & 0.58 & 0.69 & 0.64 && 0.50 & 0.46 & 0.65 & 0.54 \\
{\name} (Ours)       & 1.00 & 0.84 & 0.94 & 0.93 && 0.92 & 0.80 & 0.92 & 0.88 && 0.70 & 0.62 & 0.92 & 0.75 && 0.48 & 0.45 & 0.92 & 0.62 \\
\bottomrule
\end{tabular}
}
\end{table}





\begin{table}[tb!]
\centering
% \small
\caption{
Parameter size and editing time (averaged over 100 samples) of editing three LLMs on ZsRE. 
ROME, MEMIT, and GRACE do not contain pre-specified learnable parameters so we omit these statistics. 
Experiments were conducted on a 32-GB NVIDIA V100 GPU. 
}
\label{tab:stat}
% \renewcommand{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%{}
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{2}{c}{LLaMA 2-7b/LLaMA 2-7b-chat} && \multicolumn{2}{c}{LLaMA 3-8b-Instruct}  && \multicolumn{2}{c}{Gemma 1.1-7b-Instruct}  \\

\cmidrule{2-10}
% \midrule
                & \# Params.    & Time (sec./edit) && \# Params.    & Time (sec./edit) && \# Params.    & Time (sec./edit) \\
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-10}
AdaLoRA         & 6,292,224     & 26.24 && 5,112,576    & 28.71 && 4,817,568    & 44.24 \\
FT-L            & 45,088,768    & 9.73  && 58,720,256   & 10.84 && 75,497,472   & 11.95 \\
ROME            & /             & 27.27 && /            & 25.01 && /            & 52.07 \\
MEMIT           & /             & 20.01 && /            & 25.35 && /            & /     \\
GRACE           & /             & 34.38 && /            & 87.08 && /            & 43.45 \\
WISE\sub{light} & 5,636,096     & 58.00 && 7,340,032    & 65.77 && 9,437,184    & 20.20 \\
\cdashline{2-10}\noalign{\vskip 0.5ex}
ReFT            & 393,264       & 13.46 && 393,264      & 9.33  && 294,960      &  7.79 \\
{\name} (Ours)  & 606,256       & 10.99 && 606,256      & 12.69 && 454,704      & 10.13 \\


\bottomrule
\end{tabular}
}
\end{table}





\textbf{Batched Editing Performance.} 
We further compare {\name} and ReFT against baseline methods that \textit{admit} batched data for editing, namely, AdaLoRA, FT-L, and MEMIT. 
As in Continual Editing, three LMs are edited on ZsRE dataset, and batch sizes were set to 10 and 50 respectively. 

We present the average of reliability, generality, and locality in Fig \ref{fig:batch}, and defer the complete table to Appendix \ref{app:exp}. The proposed {\name} again achieved an excellent balance between high edit success and good locality, outperforming existing baselines in nearly all cases. 
In addition, the performance degradation compared to the pure Continual Editing is minimal.
Surprisingly, we note that when $T=10$, LoRA and MEMIT are capable of benefiting from editing multiple samples in a batch than one by one. We conjecture that learning multiple pieces of knowledge in a batch help mitigate overfitting of algorithm on any particular sample, thereby weakening the forgetting problem to some extent. This finding suggests that caching more knowledge and editing them in a batch can be beneficial in execution. 

% As a consequence,  practical continual editing, 




\textbf{Parameter Efficiency.}
Continual and Batched Editing involve learning more knowledge than in Single Editing. 
Therefore, achieving good editing performance while maintaining high parameter efficiency is non-trivial, as using fewer parameters increases the workload of each parameter to \textit{learn} more knowledge. 
When comparing {\name} with WISE on LLaMA 2-7b, lightweight WISE's editing performance dropped from 0.77 to 0.49 when editing 1000 pieces of knowledge,
around 15\% and 22\% lower than ReFT and {\name} that contain 10 times less parameters, as per Table \ref{tab:stat}. Similar trends can be found when making comparison with LoRA in Batched Editing scenarios. 
In conclusion, {\name} and ReFT are capable of achieving much better parameter efficiency than all existing methods. 


% \begin{figure}[t!]
%     \captionsetup{font=footnotesize}
%     \def\figwidth{0.3\linewidth}
%     \centering
%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}
%     %
%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}

%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}

%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}
%     %
%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}

%     \begin{minipage}[b]{\figwidth}
%     \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
%     \caption{\footnotesize Effect of Fine-tuning}
%     \label{fig::b10-llama2}
%     \end{minipage}
    
% \end{figure}

\begin{figure}[t!]
    \captionsetup[subfigure]{font=footnotesize,labelformat=parens,labelfont=footnotesize}
    % \captionsetup{font=footnotesize}
    \def\subfigwidth{0.32\linewidth}
    \centering
    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b10_llama2.pdf}
        \caption{\footnotesize LLaMA 2-7b}
        \label{fig:subfig-a}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b10_llama3.pdf}
        \caption{\footnotesize LLaMA 3-8b-Instruct}
        \label{fig:subfig-b}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b10_gemma.pdf}
        \caption{\footnotesize Gemma 1.1-7b-Instruct}
        \label{fig:subfig-c}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b50_llama2.pdf}
        \caption{\footnotesize LLaMA 2-7b}
        \label{fig:subfig-d}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b50_llama3.pdf}
        \caption{\footnotesize LLaMA 3-8b-Instruct}
        \label{fig:subfig-e}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{\subfigwidth}
        \includegraphics[width=\linewidth]{figures/b50_gemma.pdf}
        \caption{\footnotesize Gemma 1.1-7b-Instruct}
        \label{fig:subfig-f}
    \end{subfigure}

    \caption{
    Batched Editing Performance under different sequence length. The first row uses batch size 10 and the second row uses batch size 50. The proposed {\name} is capable of outperforming baselines at better parameter efficiency. 
    }
    \label{fig:batch}
\end{figure}









\subsection{Ablation Study}


% We end up this section with an ablation study on the proposed {\name}
% % with editing LLaMA 2-7b on ZsRE with $T=100$. 
% to showcase how each component contributes to its performance. 
% Results from continually editing LLaMA 2-7b with \tc{100 ZsRE knowledge} are presented in Tab \ref{tab:ablation}. 
% We note that introducing a coarse-grained subspace-level weighting (``ss-$w$ which learns one weight for the whole subspace) along did not benefit ReFT. 
% Moreover, both locality regularization (``lr'')  and fine-grained basis-level weighting (``ba-$w$'') improved locality. 
% Remarkably, the latter, as observed in all Single Editing scenarios, did not lead to edit performance degradation. 
% The former, while greatly improved the locality, degraded editing performance at the same time. 
% Such degradation is amplified when the subspace-level weighting was used. 



We end up this section with an ablation study on the proposed {\name}
% with editing LLaMA 2-7b on ZsRE with $T=100$. 
to showcase how each component contributes to its performance. 
Results from continually editing LLaMA 2-7b with 100 ZsRE knowledge are presented in Tab \ref{tab:ablation}. 
We note that introducing a coarse-grained subspace-level weighting (``ss-$w$''  which learns one weight for the whole subspace) along did not benefit ReFT. 
Moreover, both locality regularization (``lr'')  and fine-grained basis-level weighting (``ba-$w$'') improved locality. 
Remarkably, the latter, as observed in all Single Editing scenarios, did not lead to edit performance degradation. 
The former, while greatly improved the locality, degraded editing performance at the same time. 
Such degradation is amplified when the subspace-level weighting was used. 


In conclusion, the proposed {\name} makes two improvements over ReFT. 
First, the weighting offers a fine-grained level learning, leading to better locality without hurting editing performance. 
Second, a fine-grained basis-level control allows one to regularize locality by altering only the important parts, leading to a better empirical editing-locality trade-off. 

% \begin{minipage}{0.45\textwidth}
% \centering
% \begin{table}[H]
% \centering
% \caption{
%     Effect of different components in {\name}. 
%     ``\textit{ss- /ba-$w$}'': {subspace- /basis-level weight}; ``\textit{lr}'': {locality regularization}.
% }
% \label{tab:ablation}
% \resizebox{0.9\linewidth}{!}{%{}
% \begin{tabular}{r cccc}
% \toprule        
%                         & Rel.  & Gen. & Loc. & Avg. \\
% \cmidrule{2-5}
% ReFT                    & 0.76 & 0.71 & 0.84 & 0.77  \\
% \cdashline{2-5}\noalign{\vskip 0.5ex}
% \textit{+ ss-$w$}       & 0.74 & 0.68 & 0.81 & 0.74 \\
% \textit{+ ba-$w$}       & 0.77  & 0.71 & 0.86 & 0.78 \\
% \textit{+ ss-$w$, lr}   & 0.67 & 0.61 & 0.99 & 0.76 \\
% \cdashline{2-5}\noalign{\vskip 0.5ex}
% {\name}                 & 0.73  & 0.67 & 0.98 & 0.79 \\

% % ReFT                    & 0.68 & 0.61 & 0.74 & 0.68   \\
% % \cdashline{2-5}\noalign{\vskip 0.5ex}
% % \textit{+ ss-$w$}       & 0.70 & 0.65 & 0.79 & 0.71 \\
% % \textit{+ ba-$w$}       & 0.68 & 0.64 & 0.79 & 0.70 \\
% % \textit{+ ss-$w$, lr}   & 0.63 & 0.57 & 0.94 & 0.71 \\
% % \cdashline{2-5}\noalign{\vskip 0.5ex}
% % {\name}                 & 0.70 & 0.64 & 0.93 & 0.76 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
% \end{minipage}
% %
% \hfill
% %
% \begin{minipage}{0.5\textwidth}
%     \centering
%     \begin{figure}[H]
%         \centering
%         \includegraphics[width=\textwidth]{figures/weft_act.pdf}
%         \caption{Your figure caption}
%         \label{fig:yourfigurelabel}
%     \end{figure}
% \end{minipage}




\begin{wraptable}{r}{0.45\textwidth}
\centering
\caption{
    Effect of different components in {\name}. 
    ``\textit{ss- /ba-$w$}'': {subspace- /basis-level weight}; ``\textit{lr}'': {locality regularization}.
}
\label{tab:ablation}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{r cccc}
\toprule        
                        & Rel.  & Gen. & Loc. & Avg. \\
\cmidrule{2-5}
ReFT                    & 0.76 & 0.71 & 0.84 & 0.77  \\
\cdashline{2-5}\noalign{\vskip 0.5ex}
\textit{+ ss-$w$}       & 0.74 & 0.68 & 0.81 & 0.74 \\
\textit{+ ba-$w$}       & 0.77  & 0.71 & 0.86 & 0.78 \\
\textit{+ ss-$w$, lr}   & 0.67 & 0.61 & 0.99 & 0.76 \\
\cdashline{2-5}\noalign{\vskip 0.5ex}
{\name}                 & 0.73  & 0.67 & 0.98 & 0.79 \\
\bottomrule
\end{tabular}
}
\end{wraptable}

% Figure
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/weft_act.pdf}
    \caption{Your figure caption}
    \label{fig:yourfigurelabel}
\end{wrapfigure}



% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%     \centering
%     \caption{
%         Effect of different components in {\name}. 
%         ``\textit{ss- /ba-$w$}'': \textit{subspace- /basis-level weight}; ``\textit{lr}'': \textit{locality regularization}.
%     }
%     \label{tab:ablation}
%     \begin{tabular}{r cccc}
%     \toprule        
%                                 & Rel.  & Gen. & Loc. & Avg. \\
%         \cmidrule{2-5}
%         ReFT                    & 0.76 & 0.71 & 0.84 & 0.77  \\
%         \cdashline{2-5}\noalign{\vskip 0.5ex}
%         \textit{+ ss-$w$}       & 0.74 & 0.68 & 0.81 & 0.74 \\
%         \textit{+ ba-$w$}       & 0.77  & 0.71 & 0.86 & 0.78 \\
%         \textit{+ ss-$w$, lr}   & 0.67 & 0.61 & 0.99 & 0.76 \\
%         \cdashline{2-5}\noalign{\vskip 0.5ex}
%         {\name}                 & 0.73  & 0.67 & 0.98 & 0.79 \\
%         \bottomrule
%     \end{tabular}
%     \end{minipage}
%     %
%     \hfill
%     %
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/b10_gemma.pdf}
%         \caption{Your figure caption}
%     \end{minipage}
% \end{figure}



% See above results at:  /mnt/fsx/liutianc/experiments/edit-new/outputs/zsre-new/Llama-2-7b-hf_SMeFT(R=12K=1W=learn)_N=100L=100B=1S=100R=T.json
% [POST]  {'rewrite_acc': 0.671, 'rephrase_acc': 0.614, 'locality': 0.989, 'portability': 0.606, 'fluency': nan}


% See above results at:  /mnt/fsx/liutianc/experiments/edit-new/outputs/zsre-new/Llama-2-7b-hf_SMeFT(R=1K=12W=learn)_N=100L=0B=1S=100R=T.json
% [POST]  {'rewrite_acc': 0.767, 'rephrase_acc': 0.714, 'locality': 0.859, 'portability': 0.648, 'fluency': nan}


% See above results at:  /mnt/fsx/liutianc/experiments/edit-new/outputs/zsre-new/Llama-2-7b-hf_SMeFT(R=1K=12W=learn)_N=100L=100B=1S=100R=T.json
% [POST]  {'rewrite_acc': 0.728, 'rephrase_acc': 0.671, 'locality': 0.976, 'portability': 0.648, 'fluency': nan}



% See above results at:  /mnt/fsx/liutianc/experiments/edit-new/outputs/zsre-new/Llama-2-7b-hf_SMeFT(R=1K=12W=reft)_N=100L=100B=1S=100R=T.json
% [POST]  {'rewrite_acc': 0.764, 'rephrase_acc': 0.706, 'locality': 0.839, 'portability': 0.644, 'fluency': nan}




% As shown in Table \ref{tab:main},  our method achieved highly competitive performance, showing remarkable effectiveness in both batched and sequential editing scenarios. 
% In particular, comparing with MEMIT, a representative method that is specialized for batched editing, our method achieved competitive performance on the standard batched editing ($T=1$) and never encountered the catastrophic failure as MEMIT did in sequential editing. 
% Moreover, in sequential editing scenarios, our method achieved much slower performance degradation than most of existing baselines. Notably, our method contains 30 times less parameters than WISE, and does not require a separate activation routing mechanism. By comparing our method against a smaller WISE with same learnable parameter numbers, our method achieved much better parameter efficiency. 

% Finally, we note that a variety of methods achieved better editing performance on batched data than handling them separately in a sequential manner. For instance, MEMIT, ReFT, and our method all achieved better performance on editing 100 pieces of knowledge in a batch than in sequence: MEMIT achieved averaged score 0.85 on in a fully batched setting, in contrast, when editing them in sequence, the averaged score dropped to 0.03. Based on this result, we advocate that for practical benefit, it is beneficial to collect as much knowledge to edit as possible before launching an edit. 




% \begin{table}[htbp]
% \centering
% % \small
% \caption{Main editing results for QA setting (ZsRE dataset). $T$: Num Edits. WISE has much more computational resource than other methods. For a fair comparison, we restrict its capacity to the same level as ours and report these results in WISE$^*$. 
% }
% \label{tab:main}
% \resizebox{\linewidth}{!}{%{}
% \begin{tabular}{l|cccc|cccc|cccc|cccc}
% \toprule
% & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. \\
% \midrule
% % \multicolumn{17}{c}{LLaMA-2-7B} \\
% % \midrule

% \multicolumn{17}{c}{LLaMA 2-7b} \\
% \midrule
% & \multicolumn{4}{c|}{$T = 1$} & \multicolumn{4}{c|}{$T = 10$} & \multicolumn{4}{c|}{$T = 100$} & \multicolumn{4}{c}{$T = 1000$} \\
% \midrule
% FT-L & 0.57 & 0.52 & 0.96 & 0.68 & 0.48 & 0.48 & 0.76 & 0.57 & 0.30 & 0.27 & 0.23 & 0.27 & 0.19 & 0.16 & 0.03 & 0.13 \\
% % \color{red} FT-EWC & 0.96 & 0.95 & 0.02 & 0.64 & 0.82 & 0.76 & 0.01 & 0.53 & 0.83 & 0.74 & 0.08 & 0.55 & 0.76 & 0.69 & 0.08 & 0.51 \\
% LoRA & 1.0 & 0.90 & 0.92 & 0.94 & 0.39 & 0.38 & 0.50 & 0.42 & 0.06 & 0.06 & 0.06 & 0.06 & 0.00 & 0.00 & 0.00 & 0.00 \\
% MEND & 0.95 & 0.93 & 0.98 & 0.95 & 0.26 & 0.28 & 0.28 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  & 0.00 & 0.00 & 0.00 \\
% ROME & 0.96 & 0.91 & 0.98 & 0.95 & 0.38 & 0.35 & 0.05 & 0.26 & 0.18 & 0.17 & 0.02 & 0.12 & 0.01  & 0.01 & 0.00 & 0.01 \\
% MEMIT & 0.95 & 0.90 & 0.99 & 0.95 & 0.11 & 0.11 & 0.06 & 0.09 & 0.04 & 0.04 & 0.02 & 0.03 & 0.04 & 0.04 & 0.02 & 0.03 \\
% % MEMIT-MASS & 0.84 & 0.81 & 0.99 & 0.88 & 0.75 & 0.72 & 0.97 & 0.81 & 0.76 & 0.68 & 0.85 & 0.76 & 0.69 & 0.65 & 0.62 & 0.65 \\
% DEFER & 0.68 & 0.58 & 0.56 & 0.61 & 0.65 & 0.47 & 0.36 & 0.49 & 0.20 & 0.12 & 0.27 & 0.20 & 0.03 & 0.03 & 0.74 & 0.27 \\
% GRACE & 0.98 & 0.08 & 1.00 & 0.69 & 0.96 & 0.00 & 1.00 & 0.65 & 0.96 & 0.00 & 1.00 & 0.65 & 0.97 & 0.08 & 1.00 & 0.68 \\
% WISE & 0.98 & 0.92 & 1.00 & 0.97 & 0.94 & 0.88 & 1.00 & 0.94 & 0.90 & 0.81 & 1.00 & 0.90 & 0.77 & 0.72 & 1.00 & 0.83 \\
% WISE$^*$ & 0.89 & 0.61 & 0.99 & 0.83 & 0.64 & 0.58 & 0.97 & 0.73 & 0.53 & 0.49 & 0.94 & 0.65 & 0.42 & 0.41 & 0.92 & 0.58 \\
% ReFT & 1.0 & 0.99 & 0.90 & 0.96 & 0.82 & 0.80 & 0.84 & 0.82 & 0.60 & 0.67 & 0.77 & 0.68 & 0.58 & 0.57 & 0.57 & 0.57 \\
% \midrule
% Ours & 1.0 & 0.97 & 0.96 & 0.97 & 0.88 & 0.84 & 0.96 & 0.89 & 0.77 & 0.73 & 0.94 & 0.81 & 0.61 & 0.59 & 0.92 & 0.71 \\
% \midrule


% \bottomrule
% \end{tabular}
% }
% \end{table}


 % \subsection{Batched Editing Performance}



% \subsection{Sequential Editing}

% In this section we compare the proposed method against baselines in scenarios where knowledge arrives one by one. This is the standard lifelong editing setting. 

% As shown in the first block of Table \ref{tab:seq}, our method achieved highly competitive performance, showing remarkable effectiveness in sequential editing scenarios. Notably, our method contains 70 times less parameters than WISE, and it does not require a separate activation routing mechanism. 




% \begin{table}[htbp]
% \centering
% % \small
% \caption{Main editing results for QA setting (ZsRE dataset). $T$: Num Edits. WISE has much more computational resource than other methods. For a fair comparison, we restrict its capacity to the same level as ours and report these results in WISE$^*$. 
% }
% \label{tab:seq}
% \resizebox{\linewidth}{!}{%{}
% \begin{tabular}{l|cccc|cccc|cccc|cccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{4}{c|}{$T = 1$} & \multicolumn{4}{c|}{$T = 10$} & \multicolumn{4}{c|}{$T = 100$} & \multicolumn{4}{c}{$T = 1000$} \\
% & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. \\
% \midrule
% \multicolumn{17}{c}{LLaMA-2-7B} \\
% \midrule

% FT-L & 0.57 & 0.52 & 0.96 & 0.68 & 0.48 & 0.48 & 0.76 & 0.57 & 0.30 & 0.27 & 0.23 & 0.27 & 0.19 & 0.16 & 0.03 & 0.13 \\
% % \color{red} FT-EWC & 0.96 & 0.95 & 0.02 & 0.64 & 0.82 & 0.76 & 0.01 & 0.53 & 0.83 & 0.74 & 0.08 & 0.55 & 0.76 & 0.69 & 0.08 & 0.51 \\
% LoRA & 1.0 & 0.90 & 0.92 & 0.94 & 0.39 & 0.38 & 0.50 & 0.42 & 0.06 & 0.06 & 0.06 & 0.06 & 0.00 & 0.00 & 0.00 & 0.00 \\
% % MEND & 0.95 & 0.93 & 0.98 & 0.95 & 0.26 & 0.28 & 0.28 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  & 0.00 & 0.00 & 0.00 \\
% ROME & 0.96 & 0.91 & 0.98 & 0.95 & 0.38 & 0.35 & 0.05 & 0.26 & 0.18 & 0.17 & 0.02 & 0.12 & 0.01  & 0.01 & 0.00 & 0.01 \\
% MEMIT & 0.95 & 0.90 & 0.99 & 0.95 & 0.11 & 0.11 & 0.06 & 0.09 & 0.04 & 0.04 & 0.02 & 0.03 & 0.04 & 0.04 & 0.02 & 0.03 \\
% % MEMIT-MASS & 0.84 & 0.81 & 0.99 & 0.88 & 0.75 & 0.72 & 0.97 & 0.81 & 0.76 & 0.68 & 0.85 & 0.76 & 0.69 & 0.65 & 0.62 & 0.65 \\
% DEFER & 0.68 & 0.58 & 0.56 & 0.61 & 0.65 & 0.47 & 0.36 & 0.49 & 0.20 & 0.12 & 0.27 & 0.20 & 0.03 & 0.03 & 0.74 & 0.27 \\
% GRACE & 0.98 & 0.08 & 1.00 & 0.69 & 0.96 & 0.00 & 1.00 & 0.65 & 0.96 & 0.00 & 1.00 & 0.65 & 0.97 & 0.08 & 1.00 & 0.68 \\
% WISE & 0.98 & 0.92 & 1.00 & 0.97 & 0.94 & 0.88 & 1.00 & 0.94 & 0.90 & 0.81 & 1.00 & 0.90 & 0.77 & 0.72 & 1.00 & 0.83 \\
% WISE$^*$ & 0.89 & 0.61 & 0.99 & 0.83 & 0.64 & 0.58 & 0.97 & 0.73 & 0.53 & 0.49 & 0.94 & 0.65 & 0.42 & 0.41 & 0.92 & 0.58 \\
% ReFT & 1.0 & 0.99 & 0.90 & 0.96 & 0.82 & 0.80 & 0.84 & 0.82 & 0.60 & 0.67 & 0.77 & 0.68 & 0.58 & 0.57 & 0.57 & 0.57 \\
% \midrule
% Ours & 1.0 & 0.96 & 0.96 & 0.97 & 0.88 & 0.85 & 0.96 & 0.90 & 0.77 & 0.74 & 0.95 & 0.82 & 0.64 & 0.62 & 0.93 & 0.73 \\
% \midrule
% \multicolumn{17}{c}{Mistral-7B} \\
% \midrule
% FT-L & 0.58 & 0.54 & 0.91 & 0.68 & 0.39 & 0.39 & 0.50 & 0.43 & 0.11 & 0.10 & 0.02 & 0.08 & 0.16 & 0.13 & 0.01 & 0.10 \\
% % FT-EWC & 1.00 & 0.99 & 0.01 & 0.67 & 0.84 & 0.78 & 0.02 & 0.55 & 0.82 & 0.72 & 0.09 & 0.54 & 0.76 & 0.69 & 0.09 & 0.51 \\
% \color{red} LoRA \\
% % MEND & 0.94 & 0.93 & 0.98 & 0.95 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% ROME & 0.79 & 0.77 & 0.98 & 0.85 & 0.58 & 0.57 & 0.75 & 0.63 & 0.05 & 0.05 & 0.02 & 0.04 & 0.04 & 0.04 & 0.02 & 0.03 \\
% MEMIT & 0.81 & 0.79 & 0.99 & 0.86 & 0.46 & 0.45 & 0.61 & 0.51 & 0.00 & 0.00 & 0.01 & 0.00 & 0.04 & 0.04 & 0.02 & 0.03 \\
% % MEMIT-MASS & 0.81 & 0.79 & 0.99 & 0.86 & 0.74 & 0.71 & 0.97 & 0.81 & 0.73 & 0.71 & 0.88 & 0.77 & 0.73 & 0.70 & 0.62 & 0.68 \\
% DEFER & 0.64 & 0.54 & 0.79 & 0.66 & 0.53 & 0.43 & 0.29 & 0.42 & 0.28 & 0.17 & 0.26 & 0.24 & 0.02 & 0.02 & 0.67 & 0.24 \\
% GRACE & 1.00 & 0.00 & 1.00 & 0.67 & 1.00 & 0.00 & 1.00 & 0.67 & 1.00 & 0.00 & 1.00 & 0.67 & 1.00 & 0.02 & 1.00 & 0.67 \\
% WISE & 0.98 & 0.97 & 1.00 & 0.98 & 0.92 & 0.89 & 1.00 & 0.94 & 0.87 & 0.80 & 1.00 & 0.89 & 0.70 & 0.67 & 1.00 & 0.79 \\
% \color{red} ReFT & 1.0 & 0.99 & 0.90 & 0.96 & 0.82 & 0.80 & 0.84 & 0.82 & 0.60 & 0.67 & 0.77 & 0.68 & 0.58 & 0.57 & 0.57 & 0.57 \\
% \midrule
% \color{red} ours & 1.0 & 0.96 & 0.96 & 0.97 & 0.88 & 0.85 & 0.96 & 0.90 & 0.77 & 0.74 & 0.95 & 0.82 & 0.64 & 0.62 & 0.93 & 0.73 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \subsection{Batched Editing}



% In this section we compare the proposed method against baselines in scenarios where multiple pieces of knowledge arrives simultaneously. This is the standard batched editing setting, for example, one may want to update the most popular items in the last month or quarter. 

% Notably, some methods cannot handle batched edits, such as ROME, GRACE, and WISE. This limitation comes from their fine-grained mechanism to determine where to store each single knowledge. For batched knowledge, they can only handle them one by one sequentially. 
% We report experiment results in Table \ref{tab:bsz}.

% According to the table, our method again achieved remarkable performance compared to different baselines. In addition, we noted that most methods, including ours, can benefit from handling knowledge in batches than in sequences. For instance, our method 


% \begin{table}[htbp]
% \centering
% % \small
% \caption{Main editing results for QA setting (ZsRE dataset). $T$: Num Edits. WISE has much more computational resource than other methods. For a fair comparison, we restrict its capacity to the same level as ours and report these results in WISE$^*$. 
% }
% \label{tab:bsz}
% \resizebox{\linewidth}{!}{%{}
% \begin{tabular}{l|cccc|cccc|cccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{4}{c|}{$B = 1$} & \multicolumn{4}{c|}{$B = 10$} & \multicolumn{4}{c}{$B = 100$}\\
% & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg.  \\
% \midrule
% \multicolumn{13}{c}{LLaMA-2-7B} \\
% \midrule
% FT-L & 0.57 & 0.52 & 0.96 & 0.68 & 0.43 & 0.42 & 0.87 & 0.57 & 0.38 & 0.37 & 0.59 & 0.45 \\
% % \color{red} FT-EWC & 0.96 & 0.95 & 0.02 & 0.64 & 0.82 & 0.76 & 0.01 & 0.53 & 0.83 & 0.74 & 0.08 & 0.55\\
% % {\color{red} MEND} & 0.95 & 0.93 & 0.98 & 0.95 & 0.26 & 0.28 & 0.28 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 \\
% {LoRA} & 1.0 & 0.90 & 0.92 & / & 0.55 & 0.49 & 0.31 & / & 0.03 & 0.03 & 0.01 & / \\
% ROME  & 0.96 & 0.91 & 0.98 & 0.95 & 0.38 & 0.35 & 0.05 & 0.26 & 0.18 & 0.17 & 0.02 & 0.12 \\
% MEMIT & 0.95 & 0.90 & 0.99 & 0.95 & 0.89 & 0.84 & 0.97 & 0.90 & 0.87 & 0.82 & 0.87 & 0.85 \\
% % {\color{red} MEMIT-MASS} & 0.84 & 0.81 & 0.99 & 0.88 & 0.75 & 0.72 & 0.97 & 0.81 & 0.76 & 0.68 & 0.85 & 0.76 \\
% DEFER & 0.68 & 0.58 & 0.56 & 0.61 & 0.65 & 0.47 & 0.36 & 0.49 & 0.20 & 0.12 & 0.27 & 0.20 \\
% GRACE & 0.98 & 0.08 & 1.00 & 0.69 & 0.96 & 0.00 & 1.00 & 0.65 & 0.96 & 0.00 & 1.00 & 0.65 \\
% WISE & 0.98 & 0.92 & 1.00 & 0.97 & 0.94 & 0.88 & 1.00 & 0.94 & 0.90 & 0.81 & 1.00 & 0.90 \\
% \color{red} WISE$^*$ & 0.89 & 0.61 & 0.99 & 0.83 & 0.64 & 0.58 & 0.97 & 0.73 & 0.53 & 0.49 & 0.94 & 0.65 \\
% % ReFT & 1.0 & 0.99 & 0.90 & / & \\
% ReFT & 1.0 & 0.99 & 0.90 & 0.96 & 0.93 & 0.86 & 0.84 & 0.88 & 0.92 & 0.81 & 0.80 & 0.84 \\
% \midrule
% Ours & 1.0 & 0.96 & 0.96 & 0.97 & 0.93 & 0.87 & 0.92 & 0.91 & 0.92 & 0.81 & 0.88 & 0.87 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \subsection{Sequential Batched Editing}


% In this section we compare the proposed method against baselines in scenarios where multiple pieces of knowledge arrives sequentially. This is the standard batched editing setting, for example, one may want to inject new Wikipedia pages to the LLM that are released on a regular basis. For methods that do not support batched edits, we treat them as sequential edits. 
% We report experiment results in Table \ref{tab:bsz}.

% \begin{table}[htbp]
% \centering
% % \small
% \caption{Main editing results for QA setting (ZsRE dataset). $T$: Num Edits. WISE has much more computational resource than other methods. For a fair comparison, we restrict its capacity to the same level as ours and report these results in WISE$^*$. 
% }
% \label{tab:main}
% \resizebox{\linewidth}{!}{%{}
% \begin{tabular}{l|cccc|cccc|cccc|cccc}
% \toprule
% & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. & Rel. & Gen. & Loc. & Avg. \\
% \midrule
% % \multicolumn{17}{c}{LLaMA-2-7B} \\
% % \midrule

% \multicolumn{17}{c}{Batch size = 1} \\
% \midrule
% & \multicolumn{4}{c|}{$T = 1$} & \multicolumn{4}{c|}{$T = 10$} & \multicolumn{4}{c|}{$T = 100$} & \multicolumn{4}{c}{$T = 1000$} \\
% \midrule
% FT-L & 0.57 & 0.52 & 0.96 & 0.68 & 0.48 & 0.48 & 0.76 & 0.57 & 0.30 & 0.27 & 0.23 & 0.27 & 0.19 & 0.16 & 0.03 & 0.13 \\
% % \color{red} FT-EWC & 0.96 & 0.95 & 0.02 & 0.64 & 0.82 & 0.76 & 0.01 & 0.53 & 0.83 & 0.74 & 0.08 & 0.55 & 0.76 & 0.69 & 0.08 & 0.51 \\
% LoRA & 1.0 & 0.90 & 0.92 & 0.94 & 0.39 & 0.38 & 0.50 & 0.42 & 0.06 & 0.06 & 0.06 & 0.06 & 0.00 & 0.00 & 0.00 & 0.00 \\
% % MEND & 0.95 & 0.93 & 0.98 & 0.95 & 0.26 & 0.28 & 0.28 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  & 0.00 & 0.00 & 0.00 \\
% ROME & 0.96 & 0.91 & 0.98 & 0.95 & 0.38 & 0.35 & 0.05 & 0.26 & 0.18 & 0.17 & 0.02 & 0.12 & 0.01  & 0.01 & 0.00 & 0.01 \\
% MEMIT & 0.95 & 0.90 & 0.99 & 0.95 & 0.11 & 0.11 & 0.06 & 0.09 & 0.04 & 0.04 & 0.02 & 0.03 & 0.04 & 0.04 & 0.02 & 0.03 \\
% % MEMIT-MASS & 0.84 & 0.81 & 0.99 & 0.88 & 0.75 & 0.72 & 0.97 & 0.81 & 0.76 & 0.68 & 0.85 & 0.76 & 0.69 & 0.65 & 0.62 & 0.65 \\
% DEFER & 0.68 & 0.58 & 0.56 & 0.61 & 0.65 & 0.47 & 0.36 & 0.49 & 0.20 & 0.12 & 0.27 & 0.20 & 0.03 & 0.03 & 0.74 & 0.27 \\
% GRACE & 0.98 & 0.08 & 1.00 & 0.69 & 0.96 & 0.00 & 1.00 & 0.65 & 0.96 & 0.00 & 1.00 & 0.65 & 0.97 & 0.08 & 1.00 & 0.68 \\
% WISE & 0.98 & 0.92 & 1.00 & 0.97 & 0.94 & 0.88 & 1.00 & 0.94 & 0.90 & 0.81 & 1.00 & 0.90 & 0.77 & 0.72 & 1.00 & 0.83 \\
% WISE$^*$ & 0.89 & 0.61 & 0.99 & 0.83 & 0.64 & 0.58 & 0.97 & 0.73 & 0.53 & 0.49 & 0.94 & 0.65 & 0.42 & 0.41 & 0.92 & 0.58 \\
% ReFT & 1.0 & 0.99 & 0.90 & 0.96 & 0.82 & 0.80 & 0.84 & 0.82 & 0.60 & 0.67 & 0.77 & 0.68 & 0.58 & 0.57 & 0.57 & 0.57 \\
% \midrule
% Ours & 1.0 & 0.97 & 0.96 & 0.97 & 0.88 & 0.84 & 0.96 & 0.89 & 0.77 & 0.73 & 0.94 & 0.81 & 0.61 & 0.59 & 0.92 & 0.71 \\
% \midrule

% \multicolumn{17}{c}{Batch size = 10} \\
% \midrule
% & \multicolumn{4}{c|}{$T = 1$} & \multicolumn{4}{c|}{$T = 10$} & \multicolumn{4}{c|}{$T = 100$} & \multicolumn{4}{c|}{/} \\
% \midrule
% % FT-L & 0.57 & 0.52 & 0.96 & 0.68 & 0.48 & 0.48 & 0.76 & 0.57 & 0.30 & 0.27 & 0.23 & 0.27 & 0.19 & 0.16 & 0.03 & 0.13 \\
% FT-L & 0.43 & 0.42 & 0.87 & 0.57 & 0.11 & 0.10 & 0.16 & 0.12 & 0.04 & 0.03 & 0.00 & 0.02 & / & / & / & /\\
% LoRA & 0.55 & 0.49 & 0.31 & 0.45 & 0.53 & 0.48 & 0.29 & 0.43 & 0.02 & 0.02 & 0.00 & 0.01 & / & / & / & /\\
% ROME & 0.38 & 0.35 & 0.05 & 0.26 & 0.18 & 0.17 & 0.02 & 0.12 & 0.01  & 0.01 & 0.00 & 0.01 & / & / & / & /\\
% MEMIT & 0.89 & 0.84 & 0.97 & 0.90 & 0.80 & 0.74 & 0.54 & 0.69 & 0.04 & 0.04 & 0.02 & 0.03 & / & / & / & /\\
% DEFER & 0.65 & 0.47 & 0.36 & 0.49 & 0.20 & 0.12 & 0.27 & 0.20 & 0.03 & 0.03 & 0.74 & 0.27 & / & / & / & /\\
% GRACE & 0.96 & 0.00 & 1.00 & 0.65 & 0.96 & 0.00 & 1.00 & 0.65 & 0.97 & 0.08 & 1.00 & 0.68 & / & / & / & /\\
% WISE & 0.94 & 0.88 & 1.00 & 0.94 & 0.90 & 0.81 & 1.00 & 0.90 & 0.77 & 0.72 & 1.00 & 0.83 & / & / & / & /\\
% WISE$^*$ & 0.64 & 0.58 & 0.97 & 0.73 & 0.53 & 0.49 & 0.94 & 0.65 & 0.42 & 0.41 & 0.92 & 0.58 & / & / & / & /\\
% ReFT & 0.93 & 0.86 & 0.84 & 0.88 & 0.91 & 0.85 & 0.83 & 0.86 & 0.63 & 0.61 & 0.78 & 0.67 & / & / & / & /\\ 
% \midrule
% Ours & 0.93 & 0.86 & 0.92 & 0.90 & 0.91 & 0.84 & 0.92 & 0.89 & 0.63 & 0.59 & 0.93 & 0.72 & / & / & / & / \\
% % Ours & 1.0 & 0.96 & 0.96 & 0.97 & 0.88 & 0.85 & 0.96 & 0.90 & 0.77 & 0.74 & 0.95 & 0.82 & 0.64 & 0.62 & 0.93 & 0.73 \\
% \midrule


 
% \multicolumn{17}{c}{Batch size = 100} \\
% \midrule
%  & \multicolumn{4}{c|}{$T = 1$} & \multicolumn{4}{c|}{$T = 10$}  & \multicolumn{4}{c|}{/}  & \multicolumn{4}{c|}{/} \\
% \midrule
% FT-L & 0.38 & 0.37 & 0.59 & 0.45 & 0.11 & 0.09 & 0.07 & 0.09 & / & / & / & / & / & / & / & /\\
% LoRA & 0.03 & 0.03 & 0.01 & 0.02 & 0.04 & 0.04 & 0.01 & 0.03 & / & / & / & / & / & / & / & /\\
% ROME & 0.18 & 0.17 & 0.02 & 0.12 & 0.01 & 0.01 & 0.00 & 0.01 & / & / & / & / & / & / & / & /\\
% MEMIT& 0.87 & 0.82 & 0.87 & 0.85 & 0.01 & 0.01 & 0.02 & 0.01 & / & / & / & / & / & / & / & /\\
% DEFER & 0.20 & 0.12 & 0.27 & 0.20 & 0.03 & 0.03 & 0.74 & 0.27 & / & / & / & / & / & / & / & /\\
% GRACE & 0.96 & 0.00 & 1.00 & 0.65 & 0.97 & 0.08 & 1.00 & 0.68 & / & / & / & / & / & / & / & /\\
% WISE  & 0.90 & 0.81 & 1.00 & 0.90 & 0.77 & 0.72 & 1.00 & 0.83 & / & / & / & / & / & / & / & /\\
% WISE$^*$ & 0.53 & 0.49 & 0.94 & 0.65 & 0.42 & 0.41 & 0.92 & 0.58 & / & / & / & / & / & / & / & / \\
% ReFT & 0.92 & 0.81 & 0.80 & 0.84 & 0.66& 0.63 & 0.76 & 0.68 & / & / & / & / & / & / & / & / \\
% \midrule
% Ours & 0.91 & 0.80 & 0.89 & 0.87 & 0.67 & 0.63 & 0.91 & 0.74 & / & / & / & / & / & / & / & / \\




% \bottomrule
% \end{tabular}
% }
% \end{table}




